Regret Analysis of Repeated Delegated Choice

We present a study on a repeated delegated choice problem, which is the first to consider an online learning variant of Kleinberg and Kleinberg, EC'18. In this model, a principal interacts repeatedly with an agent who possesses an exogenous set of solutions to search for efficient ones. Each solution can yield varying utility for both the principal and the agent, and the agent may propose a solution to maximize its own utility in a selfish manner. To mitigate this behavior, the principal announces an eligible set which screens out a certain set of solutions. The principal, however, does not have any information on the distribution of solutions in advance. Therefore, the principal dynamically announces various eligible sets to efficiently learn the distribution. The principal's objective is to minimize cumulative regret compared to the optimal eligible set in hindsight. We explore two dimensions of the problem setup, whether the agent behaves myopically or strategizes across the rounds, and whether the solutions yield deterministic or stochastic utility. Our analysis mainly characterizes some regimes under which the principal can recover the sublinear regret, thereby shedding light on the rise and fall of the repeated delegation procedure in various regimes.

==> no-regret-learner.tex <==
\section{Delegating to No-regret Agent}
The agent does not know its own payoff function, instead he runs a no-regret learning algorithm, with respect to the best-fixed action in hindsight given the history of the principal's algorithm.
First, the agent's regret is defined as follows.
\begin{definition}[Agent's regret]
    Given mechanism $M$ and agent's algorithm $\alg$, suppose that the mechanism posts eligible set $E^{(t)}$ for $t \in T$.
    Then, the agent's regret is defined by
    \begin{align*}
        \areg_T = \max_{a \in A}\parans{\sum_{t=1}^T y_a\Ind{y_a \in E^{(t)}}} - \sum_{t=1}^T y_a^{(t)}\Ind{y_a^{(t)} \in E^{(t)}}.
    \end{align*}
    An algorithm is no-regret learning algorithm if $\areg_T = o(T)$ for any mechanism $M$.
\end{definition}

\sscomment{By considering eligible set as an adversary, we should be able to have that traditional adversarial learning algorithms like EXP3 is no-regret learning algorithm. Is this correct? (if a solution is not eligible, adversary sets that action's payoff to be zero.)}

\begin{question}
    Suppose that the agent is running a no-regret learning algorithm.
    What can be obtained for the principal under deterministic/stochastic setting?
    how the principal can learn the payoff while exploiting the fact that the agent is running no-regret algo.
    \sscomment{For example, assume that agent is running $T^{\alpha}$-regret algo for some $\alpha < 1$. Principal knows $\alpha$. Discretize the interval as a function of $T,\alpha$, run ETC-like algorithm with sufficiently large exploration per each discretized interval so that one can guarantee that agent will best-respond for each discretized interval at least e.g., almost half of that rounds, (perhaps we need some assumptions here). Finding optimal interval and commit to it. For stochastic setting, how can we extend?}
    As a side note, if the principal knows the payoff in advance (which in fact is not consistent with our previous setting), \cite{deng2019strategizing} observes that the principal can obtain Stackelberg value in average even in the simultaneous game (in fact, if the agent is simply running no-regret algo, then it boils down to simultaneous game even in our problem).
    Does this result carry over to our setting? If the principal does not know the payoff in advance, this would bring more challenges?
\end{question}


\begin{question}
    Further questions are, 
    what if the agent is running a strong algorithm of no-swap-regret?
    What if the agent is running more structured algorithm of mean-based no-regret learning algorithm?
\end{question}

\begin{question}
    Further further questions are, what if there are multiple agents running no-regret algorithm?
    For example, consider a simple class of Stackelberg-bandit style of algorithms that (i) Select agent, (ii) Agent entirely chooses solution.
    This is a subclass of general mechanism that (i) Agent submits a single solution at each round, (ii) Principal chooses a winner at each round w.r.t. commited mechanism.
    Is there any separation between these two classes?
\end{question}

\begin{question}
    Best-of-many-worlds style results.
    Can we have unified algorithm to deal with all these agents?
    For example, consider a deterministic utility and some reasonable assumptions.
    We don't know the type of agent (myopic, strategic, no-regret).
    How should our algorithm be?
    E.g., \cite{bubeck2012best} unifies stochastic/adversarial bandit algorithms.
\end{question}

==> old_single_agent.tex <==
\section{OLD - Model}

\begin{example}
    Labor market would be a good example to think of. Also, our model subsumes recommender system like Youtube, and also other many real world applications.
\end{example}
In a \emph{repeated delegated search} problem,
there is a principal and a set of agents indexed by $[n] = \{1,2,\ldots, n\}$.
Each agent $i \in [n]$ is equipped with a set of arms $A_i = \{a_{i,1}, a_{i,2}, \ldots, a_{i,k_i}\}$, where $k_i$ denotes the cardinality of the set of possible arms.
Let $A = \cup_{i \in [n]}A_i$ be the set of all the arms.
At each round $t \in [T]$, a solution $a$ incurs a nonnegative random utility for the principal and the agents.
Denote by $X_a^{(t)}$ the utility random variable (r.v.) of the principal selecting the arm $a$ and $Y^{(t)}_{i,a}$ the random utility of the agent $i$ given arm $a$. In particular, if $a \notin A_i$, then $Y^{(t)}_{i,a} = 0$.
We consider a stochastic setting in which for each arm $a \in A$, the random reward follows $(X_a^{(t)}, Y_{y_i,a}^{(t)}) \sim D_{i,a}$ for some distribution $D_{i,a}$.\footnote{Alternatively, we can interpret this model in a way that at each round $t \in [T]$, each agent is exogenously given a set of arms $A_i^{(t)} =\{a^{(t)}_{i,1},a^{(t)}_{i,2},\ldots, a^{(t)}_{i,k_i}\}$ equipped with deterministic rewards, each of which is sampled from the product distribution $D_{x,a} \times D_{y_i,a}$.}
We say that the utility of agent $i$'s solution is independent if $D_{i,a}$ is a product distribution $D_{i,a} = D_{x,a} \times D_{y_i,a}$ such that $X_{a}^{(t)} \sim D_{x,a}$ and $Y_{y_i,a}^{(t)} \sim D_{y_i,a}$.
We denote by \emph{deterministic setting} if $D_{i,a}$ has a singleton support for every $i \in [n]$ and $a \in A_i$.
In particular, we assume that the agents and principal's utilities are normalized to lie in $[0,1]$, \ie the support of $X_a^{(t)}$ and $Y_{i,a}^{(t)}$ are $[0,1]$ for any $a,i,t$.
We abuse $\Omega := [0,1]$ for simplicity.

To describe the overall process of the mechanism,
\begin{enumerate}
    \item The principal first commits to a mechanism $M$ that specifies the decision rule at each time step given the agents' action.
    \item The agents respond \emph{simultaneously} at each time step.
    \item The principal observes her own utility of the submitted solutions, and commits to one of it or possibly reject all of them.
    \item Step (2) and (3) are repeated over $T$ rounds.
\end{enumerate}
Specifically, at each round $t \in [T]$, each agent $i$ chooses a subset of arms $S_i^{(t)} \subset A_i$, and submit it to the system.
Each agent $i$ can possibly \emph{randomize} their strategies by selecting a distribution over feasible subsets.
We denote the power set of a set $X$ by $2^X$, and a simplex over $X$ by $\Delta(X)$.
In this case, each agent $i$'s action belongs to $S_i^{(t)} \in \Delta(2^{A_i})$, and we abuse $\Delta_i = \Delta(2^{A_i})$ for simplicity.
Given a set of strategies $S^{(t)} = (S_i^{(t)}, S_{-i}^{(t)})$ by the agents at time $t$ and the corresponding selected arm at the round, we abuse  $y_i(S_i^{(t)}, S_{-i}^{(t)})$ to denote agent $i$'s utility given the strategies at round $t$, and  $x(S_i^{(t)},S_{-i}^{(t)})$ to denote the principal's utility.
We use $S_i = (S_i^{(t)})_{t \in [T]}$ to denote the sequence of strategies of player $i$, and similarly define $S = (S^{(t)})_{t \in [T]}$.
For simplicity, we define $A^*$ to denote a family of all finite multi-set over a set $A$.
\sscomment{We use \emph{policy} to denote the sequence of strategies, and restrict the use of strategy to denote strictly the strategy at each round.}


\paragraph{Information}
We start with a simple setup in which each agent has a full information on the utilities of his own arms at any round, \ie $X_a^{(t)}$ and $Y_{i,a}^{(t)}$ and their corresponding distributions are fully revealed to agent $i$ for any $t \in [T]$.
We denote this setup by an \emph{informed agent setting}.
Otherwise, \ie when each agent needs to learn his own utilities over the rounds, we call it a \emph{learning agent setting}.
In the informed setting, at each round, each agent chooses his action after observes the realized utilities, while this is not the case in the learning setting.
\sscomment{Informed setting is still hard.}

\krcomment{I think single-agent case of learning-setting
when agent/principal utility are not aligned is interesting while it is definitely challenging!}

\begin{conjecture}[Informal, suspicious]
    In the informed setting, there exists a mechanism that recovers the guarantees in KK'18 and HRS'23, regardless of whether each agent knows the others' distributions or not (\ie regardless of complete info / incomplete info / no info learning setting).
	In addition, this is the best possible, \ie no mechanism has an equilibrium with a better outcome for the principal. \sscomment{\eg consider a punishment mechanism described below. Does it make sense? Any relevant literature? Optimally deceiving a learning leader...? Is it well motivated?}
    \mmcomment{Principal cannot observe the utility}
\end{conjecture}

Our main focus is on the learning setting, where each agent also needs to learn the quality of their arms by receiving feedback from the mechanism throughout the repeated interactions.
We make no assumption regarding each agent's information to each other.
Indeed, it is known that there is an algorithm for each agent that achieves a good performance, namely \emph{no-regret}, regardless of whether he has any information regarding the others' arms and statistical information therein.

%we first consider a complete information setting in which each agent knows all the others' arms and corresponding utility including his own.
%We later extend this setting by considering incomplete information setting in which each agent only knows others' distributions and further learning setting with no information a priori thus learns others' utilities over the rounds.
%\sscomment{In fact, in general, even when each agent does not have any information regarding the others' distributions, there is a an algorithm for him, inspired by experts problem, which achieves no-regret, \ie even when only the utility feedback of his own is given to him.
%Thus if we consider no-regret dynamic, this assumption may be unnecessary.}

On the other hand, the principal does not have any information on the arms and corresponding agents' utility, and thus needs to learn his own utilities over the arms in efficient manner.
Importantly, we assume that the principal only observes his own utility, not the agent's utility of the selected arm.

Based on whether the principal can distinguish different arms within an agent, we here consider two types of mechanisms as follows.
\begin{definition}[Identifiable and oblivious mechanism]
    If a mechanism can identify each solution by each agent, \eg by a serial number for each solution, we call it an \emph{identifiable mechanism} (IM).
    If a mechanism cannot distinguish multiple arms from an agent but can only identify from whom the submitted arms are registered, we call it an \emph{oblivious mechanism} (OM).
\end{definition}

\sscomment{what is (practical) Motivation for each type of mechanisms?}

\begin{conjecture}[Informal]
	For	the oblivious model, agent selection mechanism is the best we can hope for.
	% This is because since the principal cannot identify solution from each agent, we cannot expect ex-post first-best regret (as below), but we should instead define another benchmark. Indeed, since the principal can only learn which "agent" proposes a good solution, probably taking expectation over the solution distribution will make us possible to obtain a good mechanism by learning good agent who yields the largest ex-ante utility of the solution.
\end{conjecture}


\paragraph{Agent's behavior}
We define several notions regarding the behavior of agents throughout multiple interactions.
We first note that if the agents do not change their strategy but commit to their original strategy given at the initial stage, our problem reduces to the standard delegated search problem of \cite{kleinberg2018delegated} and (ours).
\sscomment{Alternatively, we can restrict the mechanism to forbid the agents to change their strategy. For example, the mechanism bans (punish) any agent who changes his strategy compared to the strategy at the initial stage, by not selecting his arm at all. Natural Q: does this type of mechanism exactly recover the equilibrium in the one-shot version of game? If this is the case, why not doing so? Such a kind of non-credible threats is indeed a thing in "(infinitely) repeated Stackelberg game", although it is usually wiped out by considering a subgame perfect Nash equilibrium for one-shot Stackelberg game. (see \href{https://en.wikipedia.org/wiki/Stackelberg_competition}{here}).
However, if each agent also needs to learn his own utility of the solutions, }
\krcomment{I think this restriction may always increase principal's utility but
why would someone consider this case in repeated delegation?
what would be the point of repetition then?
I think we can put this as a small corollary
but we note that always constant strategies is not much practical.
}
\sscomment{The point is whether our problem setting allows a trivial solution. 
I agree that this is not practical, but we should "avoid" a problem setting which admits a trivial solution that is not interesting and not practical. If we just continue pursuing the problem setup which admits this kind of weird mechanism despite just being theoretically, some reviewers may bother that our theoretical setup allows a trivial solution, thus undermines the novelty of the problem setup we considered. If the above is indeed the case, we may consider changing problem setup to avoid this kind of result. I think there also will be some lesson learned if we indeed clarify this kind of obvious result.}
Instead, the agents in our model dynamically change their strategy with respect to the specification of the mechanism and the others' response, and thereby try to maximize their own long term payoff.


\sscomment{Below dynamic is only needed for the multi-agent setting.}
One of the simplest yet most representative model to capture the dynamics of players in repeated games is \emph{best-response dynamic}, defined as follows.
\begin{definition}[Best-response dynamics]
    In best-response dynamics, at each round $t \ge 2$, each agent $i$ chooses a strategy $S_i^{(t)} = \argmax_{S_i \subset \Delta_i} y_i(S_i, S_{-i}^{(t-1)})$, \ie that maximizes his utility given that the others strategies remain the same as the previous round.
    Note that initial strategies can vary.
\end{definition}
Despite its simplistic behavior, best-response dynamics is proved to be efficient for certain types of games, \eg for any finite potential game, best-response dynamics always converge to a Nash equilibrium~\cite{nisan2007algorithmic}.
\sscomment{Best response dynamic is not well-defined in the learning setting, but only in the informed setting.}
\krcomment{I think we'll focus on this stuff later.
We should have some intuitions about what happens in multi-agent case
and then see how this best-response dynamic may work there.
}

We also consider a learning agent who tries to minimize a cumulative regret throughout the entire time horizon, formally defined as follows as per \cite{blum2008regret}.

\begin{definition}[Agent's regret]
	Given a time horizon $T$, mechanism $M$, and the others' strategies $S_{-i}$, agent $i$'s regret is defined by
	\begin{align*}
		\areg_i(S_i,S_{-i},M) 
		= 
		\max_{s_i \in \Delta_i}\Ex{\sum_{t=1}^T  y_i(s_i,S_{-i}^{(t)})} - \Ex{\sum_{t=1}^T y_i(S_i^{(t)}, S_{-i}^{(t)})}.
	\end{align*}
\end{definition}
\krcomment{We need a similar definition for the single-agent case as we are dealing with this case right now.}
Note that the expectation is taken over the randomness of the utilities,
Given a mechanism $M$, we say that agent $i$ is running a no-regret algorithm $S_i$ if it satisfies $\areg(S_i, S_{-i},M) = o(T)$ for any $S_{-i}$. 
Importantly, it is widely known that there is a no-regret learning algorithm for each agent, even without any prior information on the others' distributions (CITE).

\paragraph{Principal's objective}
The principal first announces a mechanism $M$ and commits to it. Let $a_t$ be the arm selected by the mechanism at round $t$.
Define $a_{(1)},a_{(2)}, \ldots, a_{(k)}$ for $k = \sum_{i=1}^n k_i$ be the reverse order statistics on the expected mean of arms in $A$, \ie $\Ex{X_{a_{(1)}}^{(t)}} \ge \Ex{X_{a_{(2)}}^{(t)}}\ge \ldots \Ex{X_{a_{(k)}}^{(t)}}$.

Similar to the agents, the principal aims to maximize the cumulative reward, thereby minimizing the cumulative regret defined as follows.
\begin{definition}[Principal's regret]
	Given a time horizon $T$, mechanism $M$, and corresponding strategies $S$, the first-best regret (FBR) and second-best regret are defined by
	\begin{align*}
		\freg(S,M) = \Ex{\sum_{t=1}^T \max_{a \in A} X_a^{(t)} - X_{a_t}^{(t)}}
		&= 
		T\cdot \Ex{X_{a_{(1)}}^{(t)}}- \sum_{t=1}^T \Ex{X_{a_t}^{(t)}}
		\\
	\end{align*}
	Similarly, we define the second-best regret (SBR) as follows.
	\begin{align*}
		\sreg(S,M) = \Ex{\sum_{t=1}^T \max_{a \in A} X_a^{(t)} - X_{a_t}^{(t)} } 
		&= 
		T\cdot \Ex{X_{a_{(2)}}^{(t)}}- \sum_{t=1}^T \Ex{X_{a_t}^{(t)}}.
	\end{align*}
\end{definition}
\krcomment{
I think we don't need to have $X_a^{(t)}$, it is too general. Let's assume $X_a$ does not change during the time.
}
Note that if there are multiple best arms, then the above two definitions essentially coincide.
The principal's aims to find a mechanism that recovers the sublinear first-best regret, \ie $\freg = o(T)$.
However, as shown by HRS'23, it is usually impossible to recover the first-best outcome even in the one-shot game setting.
We thereby often consider the second-best regret, \ie principal aims to have $\sreg = o(T)$ depending on the problem setting.


\paragraph{Further preliminaries}
\krcomment{I think at this point we don't need these definitions.}
We present several equilibrium studied in the literature.
\begin{definition}[Nash equilibrium]
	Given a mechanism $M$, a set of strategies $S$ is called a \emph{Nash equilibrium} (NE), if $S_i$ yields
	\begin{align*}
		\Ex{y_i(S_i, S_{-i})} \ge \Ex{y_i(S_i', S_{-i})},
	\end{align*}
	for agent $i$'s any other strategy $S_i'$ given the others' strategy $S{-i}$.
\end{definition}
In mixed Nash equilibrium (MNE), each agent can play a randomized strategy and	the expectation is taken over the randomness of the strategy.
Note that the randomized strategy here should be independent of the others' strategies so that the overall strategies $S$ result in a product distribution over $\times_{i \in [n]}A_i^*$.

\begin{definition}[Correlated equilibrium]
	Given a mechanism $M$, a set of strategies $S$ is called a \emph{correlated equilibrium} (CE), if $S_i$ yields
	\begin{align*}
		\Ex{y_i(S_i, S_{-i}) \given S_i} \ge \Ex{y_i(S_i', S_{-i}) \given S_i},
	\end{align*}
	for agent $i$'s any other strategy $S_i'$ given the others' strategy $S{-i}$.
\end{definition}

\begin{definition}[Coarse correlated equilibrium]
	Given a mechanism $M$, a set of strategies $S$ is called a \emph{coarse correlated equilibrium} (CCE), if $S_i$ yields
	\begin{align*}
		\Ex{y_i(S_i, S_{-i})} \ge \Ex{y_i(S_i', S_{-i})},
	\end{align*}
	for agent $i$'s any other strategy $S_i'$ given the others' strategy $S{-i}$.
	Note that it differs to the definition of MNE in the sense that the strategies can be correlated base on some signals given by a coordinator.
\end{definition}

Furthermore, the principal can sacrifice ex-post utility by committing to an \emph{eligible set}, thereby rejecting an arm that does not belong to the eligible set.
This will play a significant role in the single-agent setting where the principal mainly aims to learn the optimal eligible set throughout repeated interactions.
This indeed increases ex-ante utility of the principal for the one-shot setting of \cite{kleinberg2018delegated} and HRS'23.

\section{OLD - Single agent}

\sscomment{Some notations - just write down here, we can merge it into model section later. We should largely re-write the model section}.
We abuse the notations by ignoring the agent index in the single agent setting.
The agent has a discount sequence $\gamma = (\gamma_1, \gamma_2, \ldots, \gamma_T)$ such that $\gamma_t \in (0,1)$ for $t \in [T]$ and is nonincreasing.
The agent's utility can then be defined as
$\sum_{t=1}^T \gamma_t y(a_t)$ where $a_t$ denotes the arm he submits at round $t$.
For $\gamma_t = \gamma$, we say that the agent is $\gamma$-discounting.
In such case, we also define $T_\gamma = T/(1-\gamma)$.
Let $F_{x,a}(v)$ be the  probability distribution function indicating the marginal probability $\Pr{X_{a}^{(t)} \le v}$, and $F_{x,a}^-(\cdot) = \Pr{X_{a}^{(t)} < v}$.
We similarly define $F_{y,a}$ and $F_{y,a}^{-}$ for the agent's utility.javascript:void(location.href='http://proxy-um.researchport.umd.edu/login?url=%27+location.href)
\sscomment{Move below adequately}
For simplicity, we use $\mathfrak{A}$ and $\mathfrak{B}$ to denote the set of all feasible policy of the principal and the agent, respectively.
We further use $\mathcal{X}$ and $\mathcal{Y}$ to denote a policy of the principal and the agent.
\sscomment{I personally think it will be better not to define random variables $X$ and $Y$, but instead use $\om$ and $\om^*$ and $x(\om)$ as we did in previous paper.}

\begin{definition}[Allocation function]
    Given a mechanism $M$ and agent's strategy $\sigma$ after observing the realization of the utility, an interim \emph{allocation function}  $f^{(t)}_{M,\sigma}$ denotes the final outcome selected by the principal at round $t$. Note that it includes a null outcome $\perp$, \ie if the principal rejects to select any arm.
\end{definition}

We define several notations which will be useful for further expositions.
At each round, after observing the realization of the arms' utilities, a myopic agent will respond with an arm that maximizes the following quantity given the mechanism $M$.

Notably, we provide a revelation principle such that any mechanism can be reduced to a single-proposal mechanism.
\begin{theorem}
	For any mechanism $M$ and agent's policy $P$, there exists a single-proposal mechanism $M'$ and corresponding agent's policy $P'$ such that $x_{M,P} \le x_{M',P'}$  and $y_{M,P} \le y_{M',P'}$.
	This further implies that $\wreg_{M'}(T) \le \wreg_M(T)$.
\end{theorem}
\begin{proof}
	For each arm $a$, consider a reward tape, a $2 \times T$ table, in which its $(1,t)$-th and $(2,t)$-th cells refer to the realized value of $X_a^{(t)}$ and $Y_a^{(t)}$.
	The utility of the game is encoded based on the reward tables such that at each round, the utility of the arm $a$ are the values in the cells $(1,t)$ and $(2,t)$ in the reward tape of that arm.
	For each random bits of the mechanism $M$ and policy $P$, the sequence of the arms $(a_t)_{t \in [T]} \in (A \cup \{\perp\})^{T}$ chosen by the mechanism will differ.
	Obviously, there exists a set of random bits of $M$ and $P$ such that it maximizes the ex-post ....
	
	Further, given a fixed random bit of the mechanism $M$ and the policy $P$, we can deterministically identify the sequence of the arms $(a_t)_{t \in[T]} \in (A \cup \{\perp\})^{T}$ chosen by the mechanism $M$.
	\sscomment{Assume a deterministic policy}
	At each round $t$, suppose that the agent plays $S^{(t)}$ deterministically based on the history $H_t$ and $(X_a^{(t)}, Y_a^{(t)})$ for $a \in A$, and the mechanism selects $a_t \in A \cup \{\perp\}$.

	Now, consider a single proposal mechanism $M'$ such that given $H_t$, it specifies that if the agent submits $S^{(t)}$, then it will deterministically choose $a_t$.
	Then, obviously TBD
\end{proof}

This essentially implies that the principal can only optimize over the eligible sets to be announced at each round, rather than searching all the feasible mechanisms at hand.
Thus, unless specified explicitly, we now focus on the single-proposal mechanism.
Further, given a single proposal mechanism, we write $x_a^{(t)}$ and $y_a^{(t)}$ to denote the eventual utility of the principal and the agent at round $t$, when the agent proposes arm $a$.

\paragraph{Best response and Stackelberg regret}
A approximate best response of the agent is defined as follows.
\begin{definition}[$\eps$-best response]
	Given a mechanism $M$ and history $H_t$, let $A_E$ be a union of the set of eligible arms given eligible set $E$, and the null outcome $\perp$.
	Then, the $\eps$-best response at round $t$ for eligible set $E$ is defined by
	\begin{align*}
		\br_\eps^{(t)}(E) = \{a \in A_E: y_a^{(t)}\ge y_{a'}^{(t)}- \eps, \forall a' \in A\}.
	\end{align*}
	If $\eps = 0$, we simply say best response and denote by $\br^{(t)}$.
\end{definition}
Whenever there are multiple arms with best response, we assume that the agent plays in favor of the principal, \ie submits the arm that maximizes the principal's utility.

Our benchmark for a mechanism is when the mechanism knows the distribution of $X_a^{(t)}$ and $Y_a^{(t)}$ in hindsight, and if the agent best responds to the principal's action, \ie the eligible set, at each round.
In this case, the optimal principal's utility can be obtained as follows.

\begin{align*}
    \br^{(t)}(M) = \argmax_{\sigma \in \Delta}y(f^{(t)}_{M,\sigma}).
\end{align*}
We also define a $\eps$-best response as follows.
\begin{align*}
    \br^{(t)}_\eps(M) = \{\sigma \in \Delta: y^{(t)}(f_{M,\sigma}) \ge y^{(t)}_{M,\sigma'} - \eps, \forall \sigma' \in \Delta\}.
\end{align*}
We say that the agent plays a $\eps$-best response policy if he $\eps$-best responds at every rounds.

We further impose the following weak assumption, which is innocuous as discussed by CITE(OUR).
\begin{assumption}[Pareto-optimal play]\label{asmpt:pareto}
	If the agent is indifferent between multiple arms given the strategy, the agent always plays the arm that maximizes the principal's utility.
\end{assumption}



In case of the one-shot setting of \cite{kleinberg2018delegated}, they essentially observe that the single agent delegated search mechanism boils down to a design of a so-called \emph{single-proposal mechanism} due to its intrinsic structural restriction stemming the fact that it does not allow any monetary transfer.
In our extension, we mainly consider a variant of the single-proposal mechanism defined as follows.
\begin{definition}[Repeated single proposal mechanism]
	In a \emph{repeated single-proposal mechanism} (RSPM), at each round $t \in [T]$, the principal commits to an eligible set $E \subset \Omega$, the agent proposes an arm $a$, and the principal accepts the arm if $X_a^{(t)} \in E$, and otherwise rejects it.
\end{definition}

In what follows, we show that we can still construct a reduction from any repeated delegated search mechanism to a RSPM with a proper choice of the eligible sets.
\begin{theorem}[Need to be proved]
	Consider any mechanism $M$ and a corresponding $\eps$-best response $\sigma$.
	Then, there exists a RSPM $M'$ and its corresponding $\eps$-best response $\sigma'$ such that its outcome is equivalent to the outcome under $M,\sigma'$.
\sscomment{Probably we should assume that the principal can also observe agent's utility at each round?}
\sscomment{If $\eps = 0$, I think it is quite a straightforward extension. If we can also prove the extended version of $\eps > 0$, we can conclude that "even with the strategic agent, we only need to investigate single-proposal mechanism", which will be very nice.}
\end{theorem}
Importantly, this not only extends the reduction of \cite{kleinberg2018delegated}, but also strengthens it in terms of the approximate best response.

%Specifically, we consider a class of thresholded eligible set $E_\tau :=\{a \in A : x(a) \ge \tau\}$ for $\tau \in [0,1]$.
%In this case, the $\eps$-best response can be presented as follows. 
%\begin{align*}
%    \br^{\eps}(E_\tau) = \{a \in A: y(a)\Ind{a \in E_\tau} \ge y(a')\Ind{a' \in E_\tau} - \eps, \forall a' \in A\}.
%\end{align*}


Given the intrinsic structural restriction on the single agent mechanism, the problem of the principal boils down to a design of eligible set in a sequential manner to maximize her own cumulative utility.
If the principal knows the distribution of the arms' utilities $F_{x,a}(\cdot)$ and $F_{y,a}(\cdot)$ for any $a \in A$ in advance, the optimal eligible set can be computed as follows.
\begin{align}
	\opt(T) = T \cdot \max_{E \subset \Omega} \Ex{x(\br(E))\Ind{\br(E) \in E}}.\label{eq:opt}
\end{align}
Note that we omit the superscript $(t)$ since the quantity inside the expectation is indifferent over the rounds.
We denote such an eligible set by $E^*$.
We write $f(\tau) = \Ex{x(\br(E_\tau))\Ind{\br(E_\tau) \in E_\tau}}$ 0.
\sscomment{todo: make the definition generic}
\sscomment{Define offline benchmark, \ie when the distributions are deterministic.}

We simply say it an optimal eligible set when $\eps = 0$ and denote by $\opt(T) = \opt^0(T)$
Note that the expectation is computed over the randomness in the agent's solutions at each round.
Importantly, the optimal benchmark accounts for the expected utility when the agent is in fact myopic.
This is indeed the strongest benchmark since the agent does not strategize over the rounds to deceive the principal.
More formally, the following theorem states that $\opt(T)$ is indeed the upper bound on the maximal utility of the principal even if she knows the

\begin{theorem}[Need to be proved]
	Suppose that the principal knows $F_{x,a}$ and $F_{y,a}$ for any $a \in A$, and the agent possibly strategize over the rounds.
	Then, the principal's utility is at most $\opt(T)$.
	\sscomment{Trivial - as strategy includes myopic}
\end{theorem}


In our setting however, the principal does not have such information in priori, but instead needs to learn over the rounds in a sample-efficient manner.
In this context, we present the benchmark in the single-agent setting as follows.
\begin{definition}[Stackelberg regret]
	Given a mechanism $M$, suppose that the agent plays $a_t$ at each round $t \in [T]$. Then, the	\emph{$\eps$-Stackelberg regret} is defined as
    \begin{align*}
        \streg_{M, \mathcal{X}}(T) = \opt(T) - \sum_{t=1}^T x(a_t),
    \end{align*}
    where $\mathcal{X}$ is the agent's policy that specifies $a_1, a_2, \ldots, a_T$ given $M$.
    We simply say Stackelberg regret if $\eps = 0$.
\end{definition}
To compare fundamental limits of achievable regrets in various settings, we define a worst-case Stackelberg regret to be
\begin{definition}[Worst-case Stackelberg regret]
	 \sscomment{make it a formal definition} Denote by $\mathfrak{B}$ the set of all feasible policy of the agent. Then, the worst-case Stackelberg regret is
	\begin{align*}
		\wstreg_{M}(T) = \max_{\mathcal{X} \in \mathfrak{B}}\streg_{M, \mathcal{X}}(T).
	\end{align*}
\end{definition}
Importantly, when we restrict the set of policy to be $\eps$-best response, we can define the following weaker notion of worst-case Stackelberg regret.
\begin{align*}
	\wstreg_M(T, \eps) = \max_{\mathcal{X} \in \mathfrak{B}^{\eps}}\streg_{M, \mathcal{X}}(T),
\end{align*}
where $\mathfrak{B}^\eps$ denotes the set of feasible policy in which the agent is restricted to play $\eps$-best response at each round.

Obviously, $\wstreg_M(T,\eps) \le \wstreg_{M}(T)$ from the definition.

Finally, we say that a mechanism $M$ is $D$-delayed if it only uses the information gained up to round $t-D$ at each round $t \in [T]$.
Note that if $t-D \le 0$, then the mechanism acts without any information gained from the previous rounds.
Intuitively, if $D$ gets larger enough, the agent with discounted utility is less incentivized to deviate from the best response at each round.
This is because the mechanism reacts to the action at the current round with a long delay, while his utility will be discounted enough to disincentivize any deviation from the best response. 
Indeed, \cite{haghtalab2022learning} shows that with a proper choice of the delay parameter, the agent's action space can be narrowed down to the space of $\eps$-best response.
\begin{proposition}[\cite{haghtalab2022learning}]
    Given $\gamma \in (0,1)$, if we set $D = \lceil T_\gamma \log(T_\gamma / \eps)\rceil$, then $D$-delayed mechanism $M$ satisfies $\wstreg_M(T) \le \wstreg_M(T, \eps)$.
\end{proposition}
Our algorithm also grounds on the techniques of \cite{haghtalab2022learning} based on the above observation.
That said, it is still not trivial to characterize the precise regret rate from $\wstreg_M^{\eps}(T)$, and how exactly to implement such a delayed policy.
Indeed, \cite{haghtalab2022learning} considers several applications including Stackelberg security games, repeated posted price mechanism, and strategic classification to exemplify the use of their frameworks.


\begin{question}
    It seems silly to repeat all the arguments of \cite{haghtalab2022learning}.
    Can we do some general reduction techniques from delegated search with a single agent to repeated posted price mechanism?
    (Note that \cite{kleinberg2018delegated} reduces the single-agent one-shot delegated search to prophet inequalities, which is in turn a posted price mechanism.
\end{question}



\subsection{Informed agent}
We start with the simplest scenario with a single agent. Each arm of the agent is equipped with a product distribution from which the utilities of his and the principal's are drawn.
In this case, we first derive the optimal eligible set explicitly.
\begin{proposition}[Not proved yet - low priority]
    The optimal eligible set that yields \eqref{eq:opt} can be obtained by the solution of the following equation.
    \begin{align*}
        E^* = \argmax_{\tau \in [0,1]} \Ex{\br(E_\tau)\Ind{\exists a \in A: X_{a}^{(t)} \ge \tau}} := \argmax_{\tau \in [0,1]}f(\tau).
    \end{align*}
\end{proposition}
\begin{proof}
    \sscomment{We should prove that the principal only needs to care about the threshold of $x(\cdot)$. Q: is it true? We can assume that the principal cannot observe any agent's utility feedback. Assuming this, probably we can provide a counterexample that if the principal restricts some utility of the agent as well, there exists a worst-case instance such that the principal's utility becomes arbitrarily bad.}
\end{proof}

Therefore, the principal needs to learn the distribution of the arms to find the optimal thresholded eligible set $E^*$.


% In this case, identifiable and oblivious mechanism basically have no difference since all the solutions are equipped with the same distribution, and the principal's objective is to minimize expected regret over the randomness in the utility the solution.
% \sscomment{Do we need to formalize it? - ignore identifiable mechanism for now. Let's focus on only learning optimal eligible set.}
% \krcomment{
% we'll need to formalize it.
% I think now it is clear for all of us.
% maybe we formalize it after the first result is achieved.}

\subsubsection{Warmup - myopic agent}
As an initial attempt, consider a myopic agent who does not strategize over the rounds, but truthfully best-respond at each round.

\begin{question}
    This setting is very similar to The value of knowing a demand curve: Bounds on regret for online posted-price auctions, FOCS'03.
    How does it differ? Can we apply similar techniques?
\end{question}
\begin{proof}
We can easily apply the upper bounds in \cite{kleinberg2003posted} to our model with myopic agents. To accomplish this, we can form a general reduction from our model to the posted price model in this work, where any mechanism in the latter achieves a similar or lower regret in our model. Let $X^{(t)}=\max_{a\in A} X_a^{(t)}$ be the maximum value of the principal's utility among the agent's arms. Now, the principal can simulate a repeated posted-price auction where the myopic buyer has valuation $X^{(t)}$ at time $t$ as follows: At each time $t$, the principal sets a threshold $\tau$ for her utility which acts as the posted price. If the agent's valuation, $X^{(t)}$ is at least $\tau$, he will propose an eligible arm to get positive utility. Otherwise, none of the agent's arms will be eligible, and he won't propose an eligible arm. The agent's actions are therefore equivalent to the actions of a buyer with valuation $X^{(t)}$ in a posted-price auction with price $\tau$: The buyer would buy the item if and only if the agent proposes an eligible solution. 

In addition, the principal's regret in each case is at most the regret of the seller in the posted-price auction: Let $a_t$ be the arm selected by the principal at round $t$. If $X^{(t)} \geq \tau$, let $X_{a_t}^{(t)}$ be the principal utility of the proposed arm. Then, the seller would have regret $X^{(t)}-\tau$, and the principal would have regret $X^{(t)}-X_{a_t}^{(t)} \leq X^{(t)}-\tau$ as $X_{a_t}^{(t)} \geq \tau$. If $X^{(t)}<\tau$, then both the seller and the principal would have regret $X^{(t)}$. 

Therefore, if the principal adopts a strategy for posted-price auctions, he can achieve the same regret upper bounds.
\sscomment{I think this is correct only for the deterministic case, \ie when the benchmark is optimal offline solution.}

\sscomment{We should also compare how the benchmarks corresponds to each other. Eq (3.1) does not correspond to the benchmark of the repeated posted price mechanism in this case, which implies that the regret analysis does not carry over.}

What we need
\begin{align*}
	\reg_{DS}^{(t)} &= \max_\tau \Ex{X(BR_\tau) \Ind{eligible}} -X_{a_t}^{(t)}\Ind{X_{a_t}^{(t)} \ge \tau_t}
	\\
	\reg_{PP}^{(t)}&= \max_\tau \Ex{\tau \Ind{X^{(t)} \ge \tau}} -\tau_t
\end{align*}

\begin{align*}
		\reg_{DS}^{(t)} \le C \cdot \reg_{PP}^{(t)}
\end{align*}
Lipschitz assumption on $\Ex{X(BR_\tau) \Ind{eligible}}$, then can we do sth like above?

\end{proof}

%\begin{proof}[Proof of the stochastic case]
%	Given the correspondence defined as above, define 
%	\begin{align*}
%		\opt_{PP} 
%		&= \max_{\tau \in [0,1]}\tau\Pr{v_t  = X^{(t)} \ge \tau} 
%		= \tau^* \Pr{X^{(t)} \ge \tau^*},
%		\\
%		\opt_{DS} 
%		&= 
%		\max_{\tau \in [0,1]}\Ex{\br_{\tau} \Ind{X^{(t)} \ge \tau}}
%		= \Ex{\br_{\tau^\star}\Ind{X^{(t)} \ge \tau^\star}}.
%	\end{align*}
%	Then, we have
%	\begin{align*}
%		\reg_{DS}^{(t)}
%		&=
%		\opt_{DS} - \Ex{X_{a_t}^{(t)}\Ind{X_{a_t}^{(t)} \ge \tau_t}}
%		\\
%		&=
%		\parans{\max_{\tau \in [0,1]}\Ex{X^{(t)} \Ind{X^{(t)} \ge \tau}}} 
%		- \Ex{X_{a_t}^{(t)}\Ind{X_{a_t}^{(t)} \ge \tau_t}}
%		\\
%		&=
%		\max_{\tau \in [0,1]}\parans{\Ex{\tau\Ind{X^{(t)} \ge \tau}} + \Ex{(X^{(t)} - \tau)\Ind{X^{(t)} \ge \tau}}}
%		- \Ex{X_{a_t}^{(t)}\Ind{X_{a_t}^{(t)} \ge \tau_t}}
%		\\
%		&\le
%		\max_{\tau \in [0,1]}\parans{\Ex{\tau\Ind{X^{(t)} \ge \tau}}} 
%		+ 
%		\max_{\tau \in [0,1]}\parans{\Ex{(X^{(t)} - \tau)\Ind{X^{(t)} \ge \tau}}}
%		- 
%		\Ex{X_{a_t}^{(t)}\Ind{X_{a_t}^{(t)} \ge \tau_t}}
%		\\
%		&=
%		\opt_{PP}
%		+ 
%		\max_{\tau \in [0,1]}\parans{\Ex{(X^{(t)} - \tau)\Ind{X^{(t)} \ge \tau}}}
%		- 
%		\Ex{X_{a_t}^{(t)}\Ind{X_{a_t}^{(t)} \ge \tau_t}}
%		\\
%		&=
%		\opt_{PP}
%		+ 
%		\max_{\tau \in [0,1]}\parans{\Ex{(X^{(t)} - \tau)\Ind{X^{(t)} \ge \tau}}}
%		- 
%		\Ex{\tau_t\Ind{X_{a_t}^{(t)} \ge \tau_t}}
%		-
%		\Ex{(X_{a_t}^{(t)} - \tau_t)\Ind{X_{a_t}^{(t)} \ge \tau_t}}
%		\\
%		&=
%		\reg_{PP}^{(t)}
%		+ 
%		\max_{\tau \in [0,1]}\parans{\Ex{(X^{(t)} - \tau)\Ind{X^{(t)} \ge \tau}}}
%		-
%		\Ex{(X_{a_t}^{(t)} - \tau_t)\Ind{X_{a_t}^{(t)} \ge \tau_t}}
%	\end{align*}
%\end{proof}




\subsubsection{Strategic agent}
Next we consider more challenging scenario in which the agent tries to strategize over the rounds.
Since we cannot assume that the agent will truthfully best-respond to the mechanism at each iteration but instead he possibly tries to deceive the mechanism by untruthfully submitting a solution, we need to design a mechanism that is more robust to the strategic behavior.

\begin{example}[Difficult instance with not Lipschitz continuous]
	Consider a $\gamma$-discounting strategic agent with two deterministic arms $a$ and $b$.
	Let $(X_a,Y_a) = (0.5, 1)$ and $(X_b, Y_b) = (0.6, \eps_\gamma)$ for $\eps_\gamma = 0.5(1-\gamma)^T$.
	A single acceptance of arm $a$ outputs the utility of $1$,  which satisfies $1 \ge 0.5\frac{1-\gamma}{1-\gamma^T} > \eps_\gamma + \gamma \eps_\gamma + \gamma^2 \eps_\gamma + \ldots + \gamma^{T-1}\eps_\gamma$.
	The RHS denotes the utility when arm $b$ is selected every rounds.
	This implies that the agent is better off by making arm $a$ selected once, instead of making arm $b$ selected all the rounds.
	Since if the agent once proposes arm $b$, there exists no merit for the principal to accept a solution with utility smaller than $0.6$, this implies that the agent will always propose arm $a$ or does not propose anything to obtain larger utility.
	Hence the linear regret is inevitable.
\end{example}

\begin{example}[Difficult instance with sparse solution]
	Given a $\gamma$-discounting agent, let $\cI_\eps$ be a single-agent problem instance with three arms $a,b$ and $c_\eps$ such that $(X_a,Y_a) = (0.1,0.9)$, $(X_b,Y_b) = (0.2,0.8)$, and $(X_c,Y_c) = (1-\eps,\eps)$.
	Note that these arms satisfy $1$-Lipschitz continuity.
	Let $\cI'$ be the same instance but arm $c_\eps$.
	In $\cI_\eps$, to ensure that the strategic agent will ever report the arm $c_\eps$, the delay of the mechanism must reach $D_\eps = \lceil{ T_\gamma \log(T_\gamma/\eps)\rceil}$ for $T_\gamma = 1/(1-\gamma)$.
	However, the mechanism cannot distinguish $\cI'$ and $\cI_\eps$ for any $\eps>0$.
	This implies that the mechanism should increase its delay arbitrarily large in order to find $c_\eps$ which is not guaranteed to exist, and hence the linear regret is inevitable.
\end{example}

\sscomment{How to make above examples formal? Some learnability? Probably we can construct some other instances, and argue that the algorithm fails for at least one of those instances}

\sscomment{Another approach will be to show that given any mechanism, a "monotone" mechanism is better - that does not enlarge the eligible set once accepted.}

The above examples motivate us to impose the following assumption.
\begin{assumption}[Locally Nonsatiated]
	A single-agent problem instance is $d$-locally nonsatiated ($d$-LNS) for some $d > 0$ if for any arm $a \in A$, there exists another arm $b \in A$ such that $d(a, b) \le d$.
	\sscomment{We may strengthen the assumption to LNS over the pareto dominant set, if needed.}
\end{assumption}

%
%This example motivates us to impose the following smoothness assumption.
%\begin{assumption}\label{ass:deter_lipscthiz}
%	$|X_a - X_b| \le L|Y_a  - Y_b|$ for any $a,b \in A$, and there exists an arm $a$ with $Y_a \ge \eps$.
%\end{assumption}




% \begin{question}
%     This setting is very similar to Learning Prices for Repeated Auctions with Strategic Buyers, NeurIPS'13.
%     The difference is that the utility of the principal and the agents are more generally modeled, while in NeurIPS'13 they are correlated by the posted price and corresponding payoffs.
%     Moreover, the principal only needs to learn buyer's valuation, but in our case, she needs to learn both own and the agent's utility distributions.
% \end{question}

% \begin{question}
%     More generally, this is relevant to Learning in Stackelberg Games with Non-myopic Agents, EC'22, except that the principal does not know own payoff for each action.
%     By assuming the principal knows own payoff function, but does not have any information regarding the agents, we probably can apply their techniques of minimally reactive learning algorithm.
%     Also they restrict the attention to $\gamma$-discounted agent, and the algorithm entirely depends on the assumption that $\gamma < 1$.
%     Their technique cannot be applied whenever $\gamma=1$, \ie with truly farsighted agent, as the delay of the algorithm will then be $\infty$, thus incurring linear regret.
% \end{question}




\paragraph{Deterministic setting}
We start with a simple setting in which each arm has a singleton support in $[0,1]$.
In this case, the principal's objective is to find the maximal thresholded eligible set under which the agent has feasible solutions.

% \begin{algorithm}
%     \SetAlgoLined
%     $l = 0$, $u=1$, $\tau = \hat{\tau} = 0$ \\
%     \While{$u-l > 1/T$}{
%     Set $\eps = (u-l)/4$ and announce a thresholded eligible set $E_\tau$ with $\tau = (l+u)/2$ \\
%     \leIf{agent submits an eligible arm}{
%     $l\gets \tau-\eps$
%     }{$u \gets \tau+\eps$}
%     Announce $E_{\hat{\tau}}$ for next $T_\gamma \log \frac{T_\gamma}{\eps}$ rounds\\
%     $\hat{\tau} \gets \max(l-\eps, 0)$
%     }
%     Announce $E_{\hat{\tau}}$ for the remaining rounds
% \caption{\textsc{IterativeSearch}}
% \end{algorithm}

\begin{algorithm}
    \SetAlgoLined
    $\tau = 0$, $\eps = 1$\\
    \While{$\eps$ > 0}{
    Announce $E_{\tau}$ for next $T_\gamma \log \frac{T_\gamma}{\eps}$ rounds\\
    \leIf{agent submits an eligible arm $(x, y)$ in the above rounds}{
        $\tau \gets x$, break;
    }{$\eps \gets \frac{\eps}{2}$}
    }
    \While{$\eps$ > 0}{
    Announce $E_{\tau}$ for next $T_\gamma \log \frac{T_\gamma}{\eps}$ rounds\\
    \leIf{agent submits an eligible arm $(x, y)$ in the above rounds}{
        $\tau \gets x$
    }{}
    $\eps \gets \eps - d$
    }
    Announce $E_{\tau}$ for the remaining rounds.
\caption{\textsc{IterativeSearch}}
\end{algorithm}

\begin{theorem}
    \textsc{IterativeSearch} under the $d$-LNS problem instance will find the optimal solution.
\end{theorem}
\begin{proof}
    We mainly use the fact that announcing $E_{\tau} := \{a | x(a) > \tau\}$
    for at least $T_\gamma \log \frac{T_\gamma}{\eps}$
    forces the strategic agent to play $\eps$-best response, thus,
    if there exists an eligible arm $a$ (i.e. $x(a) > \tau$) such that $y(a) \geq \eps$,
    then the agent will submit that arm.
    In order to find the first eligible solution,
    we keep decreasing $\eps$ by a factor of $2$ until
    $\eps$ gets smaller than the maximum utility that an agent can get.
    In this case, the $\eps$-best responding agent will propose an arm. 
    After observing an arm $(x, y)$,
    according to $d$-LNS assumption,
    we can assume that if $a$ is not the best arm of the agent that maximizes the principal's utility,
    then there exists another arm $a'$ such that $x(a') \geq x(a)$ and $y(a') \geq y(a) - d$.
    Hence, by putting the new value for $\tau$,
    we will be able to get the next solution.
    
\end{proof}

% \begin{theorem}
%     \textsc{BatchedBinarySearch} has regret $O(\log T + T_\gamma \log T_\gamma)$ for $\gamma$-discounting agent under the deterministic utility setting.
% \end{theorem}
% \begin{proof}
%     Let $a^*$ be the arm that maximizes principal's utility.
%     Let $M^*$ be the RSPM with a fixed eligible set $E^* = \{a: x(a) \ge x(a^*)\}$.
%     Obviously, $\opt(T) = x(f_{M^*,a^*})$ as the agent's best strategy under $M^*$ is to submit $a^*$ due to Assumption~\ref{asmpt:pareto}.
%     We will prove the described regret rate with respect to the optimal arm $a^*$.

%     \begin{claim}[Not proved yet]
%         The interval $[l,u]$ always contains the true value of $x(a^*)$.
%     \end{claim}
%     \begin{proof}[Proof of the claim]
%         TBD
%     \end{proof}
%     Furthermore, the interval shrinks by a factor of $3/4$ at each iteration, which implies that $\eps$ at $i$-th iteration satisfies $\eps = (\frac{3}{4})^{i}$.
%     At each iteration, given the value of $D:= T_\gamma\log(\frac{T_\gamma}{\eps})$, the agent best responds up to the utility of $\eps$ since the mechanism responds with the delay of $D$, due to Proposition~\ref{prop:haghtalab1}.
%     That is, denoting the arm of best response by $a$, the agent responds with an arm $a'$ such that $y(f^{(t)}_{M, a'}) \ge y(f^{(t)}_{M, a}) - \eps$.
%     Since the agent gets the utility of $0$ if he submits non-eligible solution while he gets $y(f^{(t)}_{M,a})$ for the best response, there is no incentive to deviate from the best response if he $\eps$-best responds to the mechanism.
%     Then the agent play $a$ due to Assumption \ref{asmpt:pareto}.
%     Hence, the mechanism accepts the solution $a$ in line $5$ at every iteration, and also in line $7$.
%     Note also that $[l,u]$ has the interval of length $4\eps$, which implies that the regret is bounded above by $4\eps$.
%     Thus, at each round in line $5$, the principal suffers a regret of $4\eps$.
%     Let $T' = \log_{4/3}T$ and use $\eps_i$ to denote the $\eps$ at $i$-th iteration.
%     The total regret can then be bounded as follows.
%     \begin{align*}
%         \wstreg_{M}(T)
%         \le
%         \wstreg_M(T, \eps)
%         &\le
%         \sum_{i=1}^{T'}\parans{1 + 4\eps_i \cdot T_\gamma (T_\gamma/\eps)}
%         \\
%         &=
%         \sum_{i=1}^{T'}\parans{1 + 4(\frac{3}{4}^i \cdot T_\gamma \log(T_\gamma \cdot (\frac{4}{3})^i)}
%         \\ 
%         &=
%         O(\log T + T_\gamma \log(T_\gamma)).
%     \end{align*}
% \end{proof}

\paragraph{Stochastic setting}
In the stochastic setting, we use the framework of \cite{kleinberg2003value} to reduce our problem to a stochastic multi-armed bandits.
To this end, we first posits the following canonical assumptions as in \cite{amin2013learning} and \cite{kleinberg2003value}.
\begin{assumption}
    $\Pr{\exists a \in A: X_{a}^{(t)} \ge \tau}$ is $L$-Lipschitz.
\end{assumption}
\begin{assumption}
    $f(\tau)$ is maximized at a unique optimum $\tau^* \in (0,1)$ with $f''(\tau^*) < 0$, and thus there exists $c_1$ and $c_2$ with $c_1(\tau^* - \tau)^2 \le f(\tau^*) - f(\tau) \le c_2(\tau^* - \tau)^2$.
\end{assumption}

\begin{theorem}[Not proved yet]
    Let $K = T^{1/4}$, $D = T_\gamma \log(L T_\gamma T)$, and $\delta = L\eps$.
    Then ALG with the parameter above achieves regret of $O\parans{(C_2+C_1^{-1})\sqrt{T \log T} + T_\gamma \log^2(LT_\gamma T)}$ against $\gamma$-discounting agents.
\end{theorem}
\begin{proof}
    The proof relies on two technical lemmas.
    The first one is the same as Lemma 4.5 in \cite{haghtalab2022learning}, and the latter is also an analogous version of Lemma 4.6 in \cite{haghtalab2022learning} with a minor problem specific modification.
    To present the lemmas, we first define a notion of $\delta$-perturbed reward.
    
    \begin{lemma}[\cite{haghtalab2022learning}]
        For $K$-armed stochastic bandits with $\delta$-perturbed rewards and $D$-delayed feedback, \textsc{SuccessiveEliminationDelayed} achieves regret $O(\sum_{\Delta_i > 0} \frac{\log T + \delta T + D \log K}{\Delta_i})$.
    \end{lemma}
    \begin{lemma}
        
    \end{lemma}
\end{proof}
    
